Security Verification of Low-Trust Architectures

Low-trust architectures work on, from the viewpoint of software, always-encrypted data, and significantly reduce the amount of hardware trust to a small software-free enclave component. In this paper, we perform a complete formal verification of a specific low-trust architecture, the Sequestered Encryption (SE) architecture, to show that the design is secure against direct data disclosures and digital side channels for all possible programs. We first define the security requirements of the ISA of SE low-trust architecture. Looking upwards, this ISA serves as an abstraction of the hardware for the software, and is used to show how any program comprising these instructions cannot leak information, including through digital side channels. Looking downwards this ISA is a specification for the hardware, and is used to define the proof obligations for any RTL implementation arising from the ISA-level security requirements. These cover both functional and digital side-channel leakage. Next, we show how these proof obligations can be successfully discharged using commercial formal verification tools. We demonstrate the efficacy of our RTL security verification technique for seven different correct and buggy implementations of the SE architecture.

==> ISA/temp.tex <==

\section{Possible Formalization Template}

The instruction set of SE differs from existing ISAs in that it defines security properties for the instructions which the hardware must faithfully execute. We will describe the security properties of the ISA in this section and propose the properties the architecture must have in order to faithfully execute programs composed of these instructions.

The SE ISA is a conservative extension of standard RISC-V instructions. At a high level, instructions in the ISA can now be grouped as secure or insecure. Secure instructions can operate on secret values and the architecture ensure they don't leak the secret during computation. On the other hand, insecure instructions should only be executed on public data and make no security guarantees when executing on secret data. To accomplish this,  we introduce a secure instruction counterpart for all insecure instructions in RISC-V except for the control-flow instructions. For the control-flow instructions, we provide a single secure instruction as a secure alternative: $\mathsf{cmov(c, x, y)}$, which is an oblivious conditional move.


The SE ISA is data oblivious, which is necessary to guarantee the security properties of SE. Intuitively, data obliviousness places the following restrictions on the behavior of instructions:

\begin{enumerate}
	\item All secure instructions don't have timing variation
	\item All secure instructions must produce secret results
	\item \yf{todo: come back and fill this out later}
\end{enumerate}

We present the full syntax of the SE ISA in Figure \ref{fig:syntax-isa}. The semantics of the SE ISA is given as a small-step operational semantics over the configuration \yf{todo}. Now, the security properties of the instructions can be expressed in a simple security type system. We present the type system in \ref{fig:type-system-isa}. 

As is usual, we first give a soundness result for the type-system presented in Figure \ref{fig:type-system-isa}.

\begin{theorem}[SE ISA Type System Soundness]
	\yf{todo}	
\end{theorem}
\begin{proof}[Proof Sketch]
	\yf{todo}
\end{proof}


The main result we will establish in this section is that well-typed programs expressed in the SE ISA have the following two properties:

\begin{enumerate}
	\item Programs expressed in the SE ISA don't have timing-side channels on secret data\label{enum:timing-goal}
	\item Programs expressed in the SE ISA don't disclose secret data to public variables\label{enum:disclosure-goal}
\end{enumerate}

We will first state the timing property (\ref{enum:timing-goal}) in the following theorem. 
\begin{theorem}[SE ISA Side-Channel Freeness]
	\yf{todo}
\end{theorem}
\begin{proof}[Proof Sketch]
	\yf{todo}
\end{proof}

Next we will state the disclosure property in the following theorem.
\begin{theorem}[SE ISA Disclosure]
	\yf{todo}
\end{theorem}
\begin{proof}[Proof Sketch]
	\yf{todo}
\end{proof}

Some of the properties stated informally will follow from the type system trivially. We will take property (\ref{enum:xxx}) as one example to demonstrate demonstrate how the type system can be used to give the proof. \yf{todo} 


%%%%% TEMP TRASH BIN %%%%%%%


\subsubsection{\rev{Ciphertexts: Sufficient Entropy // NEED TO REWRITE} }%
\label{subsub:sufficient}
Disclosure of data can also happen due to weakness in the ciphertext. To withstand cryptanalysis attacks, the ciphertexts in the system need to maintain a predetermined unit of entropy throughout the execution of the program. If each secure instruction includes sufficient entropy in the ciphertext it produces, we can lift the property to the program.   

Every ciphertext introduces a certain fixed number of bits of entropy. It is a corollary of the no disclosure argument that ciphertexts come only from two places: from the user as input to the program or from secure SE instructions. Insecure instructions can corrupt ciphertexts (\textit{e.g.}, changing some subset of the bits of a ciphertext) which also corrupts the secret, but they cannot change the entropy in the ciphertext without corrupting the secret. 
We conclude that the data will have the desired entropy bits throughout the program.

\subsubsection{\rev{Ciphertexts: Fresh Entropy // NEED TO REWRITE}}%
\label{subsub:fresh-entropy}
Similarly, if the ciphertext does not introduce fresh entropy with each new ciphertext, an attacker can leverage cryptanalysis techniques to decipher the ciphertext without secret keys. We present a small demonstrative example in Appendix \ref{appx:attack-example} where the instruction \verb|leq| reuses the source of entropy (thus failing to refresh for each new ciphertext) and the adversarial example we present deciphers the integer in 32 iterations. \sm{If this is based on something in the literature, we should cite that.} \yf{This is an example Todd and I came up with a long time ago. Not sure if giving it as an example is fair since we don't have any significant analysis or proof showing the claim holds. Not sure if there is a similar example in the literature since I'm not familiar with the space}\shibo{It's similar to binary search, we could cite binary search and also present the example}

Intuitively, freshness captures the probability of an attacker observing the same ciphertext twice; if this probability is sufficiently high, the attacker can reliably decipher any ciphertext. Assuming that all secure instructions maintain fresh entropy on each new ciphertext, we can lift the property to programs. Given a program composed of instructions from the secure ISA defined here and assuming we fix all secret inputs to the program, we expect two independent traces of the program's execution will have the same ciphertext with a probability $\leq \epsilon$ where $\epsilon$ is a sufficiently small real number. For example, for a ciphertext generated with $N$ bits of input entropy, the probability is roughly $\frac{1}{2^{N}}$%\rev{$\frac{1}{2^{\frac{N}{2}}}$}.  

